Smaller Batches, Bigger Gains? Investigating the Impact of Batch Sizes on Reinforcement Learning Based Real-World Production Scheduling

Production scheduling is an essential task in manufacturing, with Reinforcement Learning (RL) emerging as a key solution. In a previous work, RL was utilized to solve an extended permutation flow shop scheduling problem (PFSSP) for a real-world production line with two stages, linked by a central buffer. The RL agent was trained to sequence equallysized product batches to minimize setup efforts and idle times. However, the substantial impact caused by varying the size of these product batches has not yet been explored. In this follow-up study, we investigate the effects of varying batch sizes, exploring both the quality of solutions and the training dynamics of the RL agent. The results demonstrate that it is possible to methodically identify reasonable boundaries for the batch size. These boundaries are determined on one side by the increasing sample complexity associated with smaller batch sizes, and on the other side by the decreasing flexibility of the agent when dealing with larger batch sizes. This provides the practitioner the ability to make an informed decision regarding the selection of an appropriate batch size. Moreover, we introduce and investigate two new curriculum learning strategies to enable the training with small batch sizes. The findings of this work offer the potential for application in several industrial use cases with comparable scheduling problems.

==> sec/intro_DEPRECATED.tex <==

Since the publication of Google DeepMind's Atari paper \cite{Mnih2015}, Reinforcement Learning (RL) has gained significant attention in the research community over the past decade. RL, a subset of machine learning, involves training an agent to interact with its environment in an optimal way.
Beyond video games, the applicability of RL has been explored in various domains, including finance \cite{Hambly2023}, traffic signal control \cite{Mueller2023}\cite{Noaeen2022}, and robotics \cite{Brunke2022}, among others. A particularly active area of RL research has been in the field of production scheduling \cite{Wang2022}\cite{Panzer2022}. The challenges associated with production scheduling manifest in numerous forms across the manufacturing industry, and effectively addressing these challenges can significantly impact the operational costs of manufacturing enterprises \cite{herrmann2006handbook}.

%  Methods for solving PFSSPs include heuristics, numerical methods,
% and metaheuristics. In recent years, RL has attracted more
% and more attention as an alternative approach for successfully solving scheduling problems [2], [3]. 
% However, many approaches do not move beyond the academic context due
% to their abstraction from real-world requirements, as [4], [5]
% point out.

One variant of production scheduling problems is the so-called permutation flow shop scheduling problem (PFSSP) \cite{Johnson1954}, where multiple machines must process a set of jobs in a particular order. Solving the PFSSP involves changing the order of the jobs to optimize some objective, such as the makespan. In a recent study, we examined a specific type of an PFSSP that occurs in the household appliance production at the company Miele and addressed it using RL \cite{Mueller2024}.

\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{fig/simulationmodel2_updated.pdf}
    \caption{High-Level Simulation Model in SIMPY (!!) FlexSim with conceptual integration of RL from \cite{Mueller2024}}
    \label{fig:sim_model}
\end{figure}

We introduce the problem below, a comprehensive description, including its mathematical formulation as a nonlinear mixed integer program, can be found in \cite{Mueller2024}. The problem consists of two stages, a single preassembly station (PAS) and four final assembly stations (FAS), which are connected by a finite buffer, as shown schematically in Fig.\ref{fig:sim_model}. In the PAS, semi-finished products (SFPs) are produced and subsequently stored in the buffer. These SFPs are then retrieved from the buffer and assembled into a specific final product at one of the FASs.

There are eight types of SFPs. Changing the type of SFPs on the PAS causes setup effort. At each decision step, the agent selects one of these eight types to be produced next with a fixed batch size. The buffer can initially contain different types of SFPs, with a capacity limit of 2900 units. For each of the four FASs, a sequence for producing the final products is given. The required amount and types of SFPs to be produced is derived from this set of final products. We refer to each SFP of this set as a job.

The objective is to arrange the jobs in such a way that, in lexicographical order, (1) idle time in the second stage is avoided, and (2) the sum of setup efforts in the first stage is minimized. These two goals are in conflict, since minimizing the setup effort would ideally mean not changing SFP types on the PAS. However, this would not meet the demands of the FASs, resulting in idle time.
Furthermore, each station may have different shift windows and processing times, with each product being manufactured on a station at the same processing time. The planning horizon for this scheduling problem is set to one week. 

\todo{I have one major complain about this section, it does not feel like an Introduction, mora than 70 percent of the text presents information related to your experimental setup.}


% - It is a two-stage PFSSP with multiple second stage assembly stations, finite buffers, sequence dependent setup efforts and station-related shift windows.
%     Each production job comprises two sequential operations,
%     corresponding to the two consecutive stages, for manufacturing one product.
%     - As displayed in Figure 5, a single preassembly station (PAS) in the first stage fills a central buffer with semi-finished products (SFP). The SFP are limited to a
%     small set of generic types, which are afterward converted to
%     specific products. At the following order penetration point,
%     each SFP must be assigned to a predefined non-identical final
%     assembly station (FAS) in the second stage. Under consideration of a static buffer capacity limit, it is possible that the buffer initially contains a number of SFP of different types.
%     - Thus, some jobs can skip the first stage by directly assigning.
%     - a SFP from the buffer to them. As a further complication, the
%     PAS must be suitably set up for each SFP type, which leads to
%     sequence-dependent setup efforts. Moreover, the stations can
%     have different shift windows, which can have an effect on
%     the material flows. On the FAS, some jobs have predecessor
%     relationships to other jobs on the same FAS. This means
%     that they cannot be released until the predecessor jobs have
%     been completed. 
%     - Johnson [1] demonstrated that a specialization of the problem for makespan minimization without
%     sequence-dependent setup efforts, finite buffers, work shifts
%     and release conditions can be solved exactly and efficiently
%     in polynomial time. However, the approach in this form
%     cannot be applied to our extended problem, nor were we
%     able to identify suitable efficient algorithms in the existing
%     literature. Considering the given conflicting objectives and
%     further constraints, we assume that the problem is complex
%     and that traditional algorithms are unlikely to solve it within
%     an acceptable runtime.
% Our paper addresses a specific PFSSP, a so called two-stage
% PFSSP, that occurs in a household appliance production of
% Miele. A two-stage PFSSP encompasses two distinct production stages with multiple machines in at least one of the
% stages. Thus, it is not only necessary to plan the sequence
% of jobs within the first stage, but also to consider how
% this sequence affects the material flow in the second stage.
% Due to this interdependence, two-stage PFSSPs impose more
% solving difficulties than traditional PFSSPs. The concrete
% problem considers one machine in the first stage and multiple
% machines in the second stage. Moreover, it has a finite buffer
% connecting the stages, as well as sequence-dependent setup efforts in the first stage, and machine shifts. The interdependence also arises from a tradeoff between objectives: The
% goal is to minimize idle times in the second stage and the
% setup effort required for changing product types in the first
% stage. To the best of our knowledge, this problem has not yet
% been addressed in the literature.

In the previous work, we presented an RL algorithm based on techniques like action masking, curriculum learning, and reward shaping to solve this PFSSP. 
In this study, we further analyze and extend the RL solution for smaller batch sizes on the PAS. 
% - Was haben wir in dieser Arbeit gemacht:
All experiments in the previous work were conducted with a fixed batch size of 50. Reducing the batch size would increase the flexibility of the RL agent, potentially leading to better solutions. However, it is important to note that the sample complexity of the learning process increases as the agent has to make more decisions per planning horizon. In this work, we investigate how the reduction of batch sizes affects the training success and the performance of the agent.  
% - Was sind die Ergebnisse? Was ist der Impact?
The experiments show that smaller batch sizes lead to lower setup efforts with increasing training times.
% Die Ergebnisse dieser Arbeit sind aus Anwendersicht sehr relevant. Es wird detailliert aufgeführt, welcher Trade-Off zu bestimmen ist zwischen kleinerer Batch Size zur Verringerung der Setup Efforts und gleichzeitiger Erhöhung der Trainingszeiten auf der anderen Seite.
From a batch size of 10, however, training with the current curriculum is no longer successful. We therefore present two new curricula adapted to smaller batch sizes and analyze their performance.



% Darüber hinaus lassen sich die Erkenntnisse erweitern auf ähnliche Use Cases bei denen ...

==> sec/introduction_OLDALTERNATIVE.tex <==
Reinforcement Learning is a dynamic learning paradigm from the machine learning domain that has gained significant attention in the research community over the past decade. The applicability of RL has been explored in various domains including video games~\cite{Mnih2015}, traffic signal control~\cite{Mueller2023}\cite{Noaeen2022}, and robotics~\cite{Brunke2022}, among others. A particularly active area of RL research has been in the field of production scheduling~\cite{Wang2022}\cite{Panzer2022}. The challenges associated with production scheduling manifest in numerous forms across the manufacturing industry, and effectively addressing these challenges can significantly impact the operational costs of manufacturing enterprises~\cite{herrmann2006handbook}.

%  Methods for solving PFSSPs include heuristics, numerical methods,
% and metaheuristics. In recent years, RL has attracted more
% and more attention as an alternative approach for successfully solving scheduling problems [2], [3]. 
% However, many approaches do not move beyond the academic context due
% to their abstraction from real-world requirements, as [4], [5]
% point out.

One variant of production scheduling problems is the so-called permutation flow shop scheduling problem (PFSSP)~\cite{Johnson1954}, where a set of jobs must be processed in a particular sequence by multiple machines. Solving the PFSSP involves building a sequence of jobs to optimize one or multiple objectives, such as makespan or setup effort.
% or total tardiness.

In a preliminary study~\cite{Mueller2024}, RL was utilized to solve a particular PFSSP in the household appliance production at the company Miele. The production system comprises two stages: a singular preassembly station (PAS) and four final assembly stations (FAS), linked by a central, finite buffer, 
as shown schematically in Fig.\ref{fig:sim_model}. 
At the PAS, batches of semi-finished products are produced, which are then further processed into final products at the FAS. For ease of reading, the semi-finished products are referred to as products in the following. 
There are several types of products. 
The quantity and types of products required for the FAS are predetermined. A lack of products at a final assembly station at any given time leads to idle times. Additionally, changing the types of products being produced on the PAS leads to setup efforts.
The objective is to arrange a set of product batches on the PAS in such a way that, in lexicographical order, (1) idle time in the second stage is avoided, and (2) the sum of setup efforts in the first stage is minimized. These two objectives are in conflict since minimizing the setup effort would ideally mean not changing product batches on the PAS. However, this would not meet the requirements of the FAS, resulting in idle time.
% The objective is to find a sequence for a set of product batches that minimizes two conflicting metrics in a lexicographic order: first idle times at the FAS and then setup efforts at the PAS.

Although our existing RL agent outperforms a genetic algorithm, it is important to note that it schedules batches of a fixed size, manually set by process experts at the company. However, such an assumption-based batch size may not result in the best outcomes. 
% Thus, it is highly recommended, to investigate how to determine the optimal batch size situationally. 
% The larger the batch size, the less precise and potentially more inefficient the schedule becomes; conversely, the smaller the batch size, the greater the combinatorial complexity and the higher the training effort required.
% Prior to this study, we could not identify any applicable methods in the existing literature that address this practice-relevant issue of determining ideal batch sizes.
To the best of our knowledge, there are not any applicable methods in the existing literature that address this practice-relevant issue of determining ideal batch sizes.
This work proposes a systematic approach for analyzing the impact of varying batch sizes on the agent's performance. Our approach contributes to identifying the optimal batch size ("sweet spot") that balances the agent's training and scheduling efficiency. Moreover, we apply curriculum learning and introduce two new curricula tailored to smaller batch sizes, which are likely to be transferable to comparable real-world production systems. 
An interesting key finding from our experiments indicates that smaller batch sizes result in lower setup efforts but incur longer training times. However, if the batch sizes are too small, it is only possible to train an agent with good scheduling efficiency with the help of the new curricula. But this comes at the price of long training times. 
% Interestingly, the optimal sweet spot for the batch size can be quite delicate, with minor deviations potentially leading to the failure of the whole training.

\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{fig/simulationmodel2_updated.pdf}
    \caption{Abstract model of the production environment within a discrete-event simulator and the conceptual integration of RL for determining the sequence of semi-finished product batches (reprinted from Müller et. al.~\cite{Mueller2024}).}
    \label{fig:sim_model}
\end{figure}

==> sec/problem_formulation.tex <==
%\subsection{Problem Formulation}


% Input in das Optimierungsproblem: Ein Datensatz
% Output: 

% Entscheidungsvariable: Sequence von Produkttypen

% Optimierungsziele in lexikographischer Weise: Zuerst idle times in den final assembly stations minimieren und dann setup effort in der preassembly station

% Nebenbedingungen:
% - Ein Auftrag muss über beide Stationen
% - Aufträge müssen in fester Reihenfolge abgearbeitet


% OPTIMIERUNGSPROBLEM
% PFSSP
%The specific scheduling problem at hand is a so-called permutation flow shop scheduling problem (PFSSP)~\cite{Johnson1954}. 


%The input to the problem consists of a sequence for each FAS and a defined batch size for the PAS production. Each element in these sequences consists of the quantity and type of a required product at a given time step~$t$. If there is no product of the required type in the buffer at a given time step, then there will be idle times in the FAS. Furthermore, the input consists of an initial buffer allocation, so that the FAS can pull the required products from the buffer right at the beginning of the planning horizon. Otherwise, the FAS must to wait for the PAS to build the required products, which leads to idle times in the beginning. Recall that the input also consists of a batch size~$b$ specifying the production at the PAS. More precisely, the products are produced in batches of size~$b$ at the PAS. Changing the product types on the PAS leads to setup efforts. All information about setup times is encoded as a setup matrix.

% OBJECTIVES
%The objective is to find a sequence of product types for the PAS in such a way that, in lexicographical order, (1) idle time in the FAS, and (2) the sum of setup efforts in the PAS are minimized. These two objectives are in conflict since minimizing the setup effort would ideally mean not changing product types on the PAS. However, this would not meet the requirements of the FAS, resulting in idle time.





